Latent Part-of-Speech Sequences for Neural Machine Translation

Learning target side syntactic structure has been shown to improve Neural Machine Translation (NMT). However, incorporating syntax through latent variables introduces additional complexity in inference, as the models need to marginalize over the latent syntactic structures. To avoid this, models often resort to greedy search which only allows them to explore a limited portion of the latent space. In this work, we introduce a new latent variable model, LaSyn, that captures the co-dependence between syntax and semantics, while allowing for effective and efficient inference over the latent space. LaSyn decouples direct dependence between successive latent variables, which allows its decoder to exhaustively search through the latent syntactic choices, while keeping decoding speed proportional to the size of the latent variable vocabulary. We implement LaSyn by modifying a transformer-based NMT system and design a neural expectation maximization algorithm that we regularize with part-of-speech information as the latent sequences. Evaluations on four different MT tasks show that incorporating target side syntax with LaSyn improves both translation quality, and also provides an opportunity to improve diversity.

==> discard_background.tex <==
\section{Background}
\nb{Xuewen, I think you can omit this section completely. You can assume that the NLP community knows the MT problem, its formulation and is familar with EM. Whatever terminology you need can be introduced directly in what is section 3. This space can be used for describing the models and results better.}
In this section, we review Neural Machine Translation (NMT) background and EM algorithms.
\subsection{Neural Machine Translation}

Given a source sentence $\mathbf{x} = \mathbf{x}_1, \ldots, \mathbf{x}_M$ and a target sentence $\mathbf{y} = \mathbf{y}_1, \ldots, \mathbf{y}_N$, an end-to-end NMT model directly models the conditional probability:

\begin{equation}
P(\mathbf{y} \vert \mathbf{x}; \boldsymbol{\theta}) = \prod_{n=1}^{N} P(\mathbf{y}_n\vert \mathbf{x}, \mathbf{y}_{<n};\boldsymbol{\theta})
\end{equation}
where $\boldsymbol{\theta}$ is a set of model parameters and $\mathbf{y}_{<n} = \mathbf{y}_1,\ldots , \mathbf{y}_{n-1}$ is a partial translation. The training objective is to maximize the log-likelihood of the training corpus:

\begin{equation}
\begin{aligned}
\sum_{\langle \mathbf{x}, \mathbf{y} \rangle \in D}\log P(\mathbf{y} \vert \mathbf{x}; \mathbf{\theta}) 
\end{aligned}
\end{equation}
where $\langle \mathbf{x}, \mathbf{y} \rangle$ is the parallel sentence pair from the training corpus $D$.

A NMT system directly models the conditional probability with a structure consisting of two components: (a) an \textit{encoder} which computes a representation for each source sentence and (b) a \textit{decoder} which generates one target word at a time. Different structures exist for NMT \cite{Sutskever14, Gehring17, Nal16, Vaswani17}. In this paper, we select Transformer \cite{Vaswani17} as our base structure.


\subsection{EM Algorithm}
The \textit{expectation maximization} (EM) algorithm is a general iterative technique to find maximum likelihood solutions for statistical models having latent variables \cite{bishop2006}. It consists of two steps: an expectation (E) step, which calculates the expectation of the log-likelihood evaluated given the current parameters, and a maximization (M) step, which updates the parameters to maximize the expected log-likelihood found in the E step. These parameter-estimates are then used to determine the distribution of the latent variables in the next E step. 

In machine translation, many linguistic features can serve as the latent variable. In this paper, we use POS tags since they can help in language disambiguation and word re-ordering. Then we apply EM algorithm to properly integrate this latent variable. Since there is no closed form solution for the EM algorithm for NMT, we propose Neural EM (NEM) and update model parameters with Stochastic Gradient Descent.













==> old-introduction.tex <==
\section{Introduction}

Neural machine Translation (NMT) has achieved impressive results on many translation tasks in recent years \cite{BahdanauCB14, luong2015, SennrichHB16, Vaswani17} and has been proved in application to work better than general Statistical Machine Translation (SMT) models. Current NMT models generally use the encoder-decoder structure \cite{Sutskever14, Cho14} where an encoder encodes a source sentence to a sequence of latent representations, which the decoder then uses to decode the target sentence. Additionally, attention mechanism \cite{BahdanauCB14, luong2015} allows the model to focus on relevant parts of the source sequence when decoding and greatly improves the translation performance. While NMT models have made remarkable progress, they still face three problems. First, in most cases, they are trained on parallel corpus in an end-to-end way without using any other linguistic information. Exploiting other linguistic information can be crucial for translation performance and has been proven not to be redundant even though NMT models have strong learning capability. For example, POS tags are very helpful to model word re-ordering between languages and can help in language disambiguation~\cite{niehues2009}. Lemmatization can reduce data sparseness, and allow inflectional variants of the same word to explicitly share a representation in the model~\cite{SennrichHB16}. \textcolor{red}{Second, current NMT models are not explicitly interpretable and anticipated. The decoding process is kind of mysterious that follow some implicit rules. (Controllability is important? In our model, to control the model, we have to provide accurate POS tags. This information might not be available in practice. What are the scenarios that make controllability important?) Third, given some predefined translation constraints, they are not able to comply with them. For instance, for some specific words or phrases, terminology lists are often used to guide the translation process} ~\cite{chatterjee2017}. \nb{Diversity is another angle. That is controllability gives us a way to produce diverse translations for the same input. This has been motivated as a way to get N-best lists for beam rescoring or say providing for a personalized translation for a specific user.}

To solve the above problems, in this work, we exploit application of POS tags as an extra linguistic feature. The model can be extended to integrate other linguistic features similarly. 
%The intuition is that given source language, if we can infer the POS tags of target language, then we can use the inferred POS tags to guide language translation process. 
\textcolor{red}{We want the translation be generated by not only the source language, but the linguistic features of the target language, which is introduced by a latent variable $z$. Then we use the linguistic features to regularize the action of the latent variable.} The inferred POS tags can also serve as an extra feature to help improve translation quality. There exist three concerns about this intuition. First, how can we guarantee that the inferred POS tags are accurate enough? If the inferred POS tags are not accurate enough, then the error will accumulate to make the translation results even worse. Second, even tough we can infer accurate enough POS tags from source language, how well NMT can perform after having this extra feature? Third, how to infer POS tags from source language? To dispel these three concerns, we propose a novel translation model POS Tags Guided NMT (POST-NMT) and trained it with a Regularized Neural Maximization Expectation (RNEM) algorithm. The translation can then be described as an recurrent process that a POS tag is first generated from the source sentence and the previous target tokens, then the current target token is generated from this POS tag and the previous target tokens, as shown in Figure~\ref{fig:Bayes1}. This design makes sure that at every step, we only need to sample a limited number (size of POS tag vocabulary) of candidates. Different from other sampling methods where only $k$ candidates are sampled because of exponential sampling space~\cite{cheng2016, shen2016}, RNEM searches all possible candidate POS tags for each target token. This makes sure all possible candidates are considered at each time step. Thus the prediction accuracy of POS tags are improved. To further improve the POS tag prediction accuracy, in the training process, we regularized our model with groundtrue POS tags. Note that our model can be easily extended to other linguistic features as POS tags. The empirical upper bounds of translation tasks after adding accurate POS tags are also given to show that this is a path that more attention should be given on.

To demonstrate the effectiveness of the proposed POST-NMT, we evaluate our model on four translation tasks IWSLT'14 English-German, German-English, English-French and French-English. Our experiments show that (i) POS tags of target language can be predicted from source language accurately enough. (ii) POST-NMT trained with RNEM leads to significant improvements over state-of-the-art NMT systems~\cite{Vaswani17, Gehring17}. (iii) the inferred POS tags serve as a guide in the translation process, thus makes translation interpretable and anticipated to some extent.

The proposed model has three advantages: (i) POST-NMT proposes a descent way to integrate discrete linguistic hidden variables by using Regularized Neural Expectation Maximization and thus improve translation qualitiy. (ii) It makes the translation controllable by external knowledge. (iii) It alleviates the needs of doing exponential search in other general neural machine translation.





























==> scratch.tex <==

% abstract begins here
%Most prior work define syntactic information as tree structures, which complicates the inference process.
%As searching the whole space of the tree structures is almost impossible, existing models rely on greedy search strategies to explore a limited portion of it.

%In this work, we define a simpler sequential structure for the learning of the target side syntax structure to improve the translation quality and diversity. In particular, we consider the syntax as a sequence of latent variables and design an efficient network architecture that allows us to exhaustively search the whole latent space rather than only sampling from the most likely sequences. This latent space can be supervised with parts-of-speech (POS) tag information when available, but can also be entirely unsupervised. A key benefit of our method is that the network is able to produce diverse translations by exploring different parts of the latent space. 
%Extensive empirical experiments on four different translation tasks demonstrate that our model outperforms NMT methods that only use source side syntax, and some methods that use syntax information on the target side.

%We propose a new NMT model with a sequence of latent variables and devise an EM based inference strategy. 

%Existing methods on Neural Machine Translation (NMT) directly model the conditional probability $P(\mathbf{y} \vert \mathbf{x})$ of the target translation $\mathbf{y}$ given the source sentence $\mathbf{x}$. These methods do not explicitly utilize the linguistic features of the language and expect the model to learn them in an implicit way. This strategy prohibits the current methods to profit on linguistic features, which contains the most direct language structure information of a language. Besides, it is hard to have diverse translation as source sentence is given, target translations are only determined by search algorithms. To address these two problems, we propose a novel NMT model, which embeds the linguistic property of the target language through the introduction of a sequence of latent variables. We then introduce a Regularized Neural Expectation Maximization (RNEM) algorithm to address the training problem. In this paper, we define the latent states as the sequence of POS-tags, which is one of the simplest linguistic feature of translation context. Our extensive experimental results show that the proposed NMT model outperforms (or has comparable result with) the state-of-the-art methods on the five challenging translation tasks. Furthermore, our model is able to produce different meaningful translations by varying on POS-tag sequences.

% abstract ends here



% introduction begins here

% We evalaute the effectiveness of \name on four translation tasks. The evaluations highlight the two main advantages of our model: (i) Target side syntax modeled using POS tag sequences, leads to significant improvements over state-of-the-art NMT systems~\cite{Vaswani17, Gehring17}. (ii) By feeding different POS tag sequences into the model, diverse meaningful translation can be generated.





% \eat{Neural machine Translation (NMT) has achieved impressive results on many translation tasks in recent years~\cite{BahdanauCB14, luong2015, SennrichHB16, Vaswani17}. Current NMT models generally use the encoder-decoder structure~\cite{Sutskever14, Cho14} to model the conditional probability of $P(\mathbf{y} \vert \mathbf{x})$, where an encoder encodes a source sentence into a sequence of latent representations, which are then decoded into the target sentence. 
% %Additionally, attention mechanism~\cite{BahdanauCB14, luong2015} allows the model to focus on relevant parts of the source sequence when decoding and greatly improves the translation performance. 
% While remarkable progress has been made in the design of NMT models, existing approaches cannot explicitly leverage syntactic information of languages, which has been shown to be crucial for the performance of Statistical Machine Translation~\cite{Chiang2009, Huang2006, Shen2008}. Recently, some syntactic information has been exploited in NMT through three methods, incorporating the syntactic information into the source-side~\cite{Chen18Syntax, SennrichLinguistic16, eriguchi2016tree}, using multi-task learning to benefit from other tasks in machine translation~\cite{eriguchi2017learning, Baniata18, Niehues17, Zaremoodi18}, or applying the syntactic knowledge to the target side~\cite{Shu18, gu2018top, wang2018tree}. However, the first method strictly requires the availability of external tools during inference time~\cite{eriguchi2017learning}, while the second one needs careful model selection which can be non-trivial~\cite{Zhang18Learning}. Though the third method is most effective, it still has some drawbacks. They are generally similar to the graphical model in Figure~\ref{fig:Bayes2}, which use $P(\mathbf{y} \vert \mathbf{z}^{\ast},\mathbf{x})P(\mathbf{z}^{\ast} \vert \mathbf{x})$ to approximate $P(\mathbf{y} \vert \mathbf{x})$, where $\mathbf{z}$ is an observed variable representing the syntactic information of the target side, and $\mathbf{z}^{\ast}=\arg max_{\mathbf{z}} P(\mathbf{z} \vert \mathbf{x})$. This design scheme can be error prone because it can only explore a small portion of space $\mathbf{z}$ and difficult to find the optimal $\mathbf{z}^{\ast}$. Moreover, most of existing schemes utilize a complex tree structure which can be very hard to model. 

% While we use simpler part-of-speech (POS) tag sequence as the syntax structure.
% First, while they can \textit{implicitly} discover syntactic properties of the source language~\cite{shi2016string}, they do not \textit{explicitly} leverage such information. 
% they are trained on parallel corpus without explicitly using any linguistic information. 
% and has been proven not to be   redundant even though NMT models have strong learning capability. For example, POS tags are very helpful to model word re-ordering between languages and can help in language disambiguation~\cite{niehues2009}. Lemmatization can reduce data sparseness, and allow inflectional variants of the same word to explicitly share a representation in the model~\cite{SennrichHB16}. 
% Second, NMT models use beam search or other search algorithms to decode target sentences. The diversity of the translation is thus limited, while human being can make different translations for one sentence depending on the structure of the target sentence he uses~\cite{eriguchi2016tree}.
% Second, given some predefined translation constraints, they are not able to comply with them. For instance, for some specific words or phrases, terminology lists are often used to guide the translation process~\cite{chatterjee2017}. \nb{Diversity is another angle. That is controllability gives us a way to produce diverse translations for the same input. This has been motivated as a way to get N-best lists for beam rescoring or say providing for a personalized translation for a specific user.}
% To solve the first problem, recent works have established some explicit methods to leverage syntactic information in three aspects. First, through integrating syntactic information in the source-side, translation performance can be improved~\cite{Chen18Syntax, SennrichLinguistic16, eriguchi2016tree}. However, the trained translation models strictly require the availability of external tools during inference time~\cite{eriguchi2017learning}.
% Second, using multi-task learning strategy, machine translation tasks can benefit from other tasks like part-of-speech (POS) tagging, named-entity recognition, syntactic parsing or semantic parsing~\cite{eriguchi2017learning, Baniata18, Niehues17, Zaremoodi18}. The syntactic information can be added to the main translation task by jointly training with other side tasks. Nevertheless, the multi-task learning structure can be quite complex and the hyper-parameter tuning can be non-trivial.  
% The third method is by directly modeling the syntactic structure of the target side~\cite{Shu18, gu2018top, wang2018tree}. These models are generally similar to the graphical model in Figure~\ref{fig:Bayes2}, where they use $P(\mathbf{y} \vert \mathbf{z}^{\ast})\times P(\mathbf{z}^{\ast} \vert \mathbf{x})$ to approximate $P(\mathbf{y} \vert \mathbf{x})$, where $\mathbf{z}$ is an observed variable representing the syntactic structure of the target side, and $\mathbf{z}^{\ast}=\arg max_{\mathbf{z}} P(\mathbf{z} \vert \mathbf{x})$. This method can be error prone because it can only sample a small portion of space $\mathbf{z}^{\ast}$. Moreover, the complex tree structure can be very hard to predict. 
% While we use simpler part-of-speech (POS) tag sequence as the syntax structure.

% In contrast to the third method that only a small portion of $\mathbf{z}$ space can be explored, we design a novel scheme to exhaustively search full space of latent variable $\mathbf{z}$.
% The key to achieving this objective is a novel architecture design that the latent variable $\mathbf{z}_n$ at time step $n$ is inferred from source sentence $\mathbf{x}$ and partial translation $\mathbf{y}_{<n}$, but not directly from $\mathbf{z}_{<n}$, as shown in Figure~\ref{fig:Bayes3}. It is sufficient to infer an accurate $\mathbf{z}_{n}$ from $\mathbf{y}_{<n}$, as the syntactic structure is directly represented in the translation context. With this specific design of the variable dependencies, the time complexity of searching for the latent states becomes linear with respect to the length of sentence. Thus, it becomes possible to exhaustively search through the latent states and model the target distribution by $P(\mathbf{y} \vert \mathbf{x}) = \sum_{\mathbf{z}} P(\mathbf{y}, \mathbf{z} \vert \mathbf{x})$.


% To further improve the translation quality, we regularize the learning of the latent variable $\mathbf{z}$ with POS tag sequences, which is a simpler syntax knowledge than trees.
% The training of the model can be decently performed by our proposed Regularized Neural Expectation Maximization (RNEM) algorithm.
% And by sampling latent variable $\mathbf{z}$ to get different POS tag sequences, our model gives us another advantage over other methods - generating diverse translations for one source sentence. This is a more explicit and effective way of performing diverse translation than other methods based on diverse or re-ranking beam search~\cite{Vijayakumar18, LiJ16mutual}, or coarse codes planning~\cite{Shu18}.
% To solve the second problem, different methods have been proposed. Vijayakumar \textit{et al.}~\shortcite{Vijayakumar18} proposed a diverse beam search algorithm and Li \textit{et al.}~\shortcite{LiJ16mutual} proposed a re-ranking beam search method to improve the decoding diversity. Dou \textit{et al.}~\shortcite{dou2018exploiting} used a regularization term to encourage the difference between two consecutive layers and thus improve the diversity of translation. Yet, the translation diversity of these models is limited. Shu \textit{et al.}~\shortcite{Shu18} used an autoencoder to generate a coarsely short codes from which the translation is generated. However, whether this method works or not for long sentences is under-explored. In this work, we achieve this objective by sampling the latent sequence of variable $\mathbf{z}$. By sampling $\mathbf{z}$, we are generating different POS tag sequences that the sentence is generated from. As our method samples all the choices of $\mathbf{z}$, the translation quality can be guaranteed.


% To solve the above problems, in this work, we exploit application of POS tags as an extra linguistic feature. The model can be extended to integrate other linguistic features similarly. 
% The intuition is that given source language, if we can infer the POS tags of target language, then we can use the inferred POS tags to guide language translation process. 
% \textcolor{red}{We want the translation be generated by not only the source language, but the linguistic features of the target language, which is introduced by a latent variable $z$. Then we use the linguistic features to regularize the action of the latent variable.} The inferred POS tags can also serve as an extra feature to help improve translation quality. There exist three concerns about this intuition. First, how can we guarantee that the inferred POS tags are accurate enough? If the inferred POS tags are not accurate enough, then the error will accumulate to make the translation results even worse. Second, even tough we can infer accurate enough POS tags from source language, how well NMT can perform after having this extra feature? Third, how to infer POS tags from source language? To dispel these three concerns, we propose a novel translation model POS Tags Guided NMT (POST-NMT) and trained it with a Regularized Neural Maximization Expectation (RNEM) algorithm. The translation can then be described as an recurrent process that a POS tag is first generated from the source sentence and the previous target tokens, then the current target token is generated from this POS tag and the previous target tokens, as shown in Figure~\ref{fig:Bayes1}. This design makes sure that at every step, we only need to sample a limited number (size of POS tag vocabulary) of candidates. Different from other sampling methods where only $k$ candidates are sampled because of exponential sampling space~\cite{cheng2016, shen2016}, RNEM searches all possible candidate POS tags for each target token. This makes sure all possible candidates are considered at each time step. Thus the prediction accuracy of POS tags are improved. To further improve the POS tag prediction accuracy, in the training process, we regularized our model with groundtrue POS tags. Note that our model can be easily extended to other linguistic features as POS tags. The empirical upper bounds of translation tasks after adding accurate POS tags are also given to show that this is a path that more attention should be given on.

% We name our model as POS Tags guided NMT (POST-NMT). 
% To demonstrate the effectiveness of the proposed NMT model, we evaluate it on performing four translation tasks. Our extensive experiments show two advantages of our model: (i) POS tag sequence, a simple syntactic information, is well incorporated by RNEM learning algorithm, which leads to significant improvements over state-of-the-art NMT systems~\cite{Vaswani17, Gehring17}. (ii) By feeding different POS tag sequences into the model, diverse meaningful translation can be generated.

% }
% The proposed model has three advantages: (i) POST-NMT proposes a descent way to integrate discrete syntactic hidden variables by using Regularized Neural Expectation Maximization (RNEM) and thus improve translation quality. (ii) It alleviates the needs of doing exponential search in other general neural machine translation.


% introduction ends here


% model begins here
%sampling $\mathbf{z}$ involves exponential search.} 
%Sampling remains computationally expensive, even \rev{with} a restricted subset of the full space, \rev{which} also \rev{introduces} errors in both training and inference. }\note{Just for one sequence, why can't you sample? Or all possible sequences? Why sample needs search?}\xy{For a vocabulary of size V, and a sequence of length N, the total number of possible samples are $V^N$.}
%The model must use greedy or beam search decoding of $\mathbf{z}$ before decoding words.
%Our goal is to design to components that will effectively model $P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})$ and $P(\mathbf{z}_n\vert \mathbf{x}, \mathbf{y}_{<n})$.

%\nb{Xuewen, read the following lines carefully to see if this is accurate. It will be easier to follow if you can make the green oval in Figure 2 to clearly represent what it contains.}\xy{I think your writing is good. We need a third person to look at it to see whether this is clear to every one. Basically, to model $P(y_n\vert z_n)$, we have to introduce another dimension which is the dimension of z. $y_n\in \mathcal{R}^{N\times D}$ becomes $y_n\in \mathcal{R}^{N\times V_z\times D}$, this means the probability of $y_n=i$ will be spread over $z_n=1:V$. So ADDing all $z_n$ actually is calculating $P(y_n\vert z_n=1...V)$}


%The \texttt{Add} operation simply adds up the embeddings with the inter-attention outputs, which is achieved by broadcasting the embeddings and the inter-attention outputs to the same dimension and then point-wisely add them together. The final result is then fed to linear transform and softmax over the target word vocabulary, %\nb{Xuewen, can you write a sentence or two here that explains why this way of concatenating embeddings can be seen as conditioning on different choices of $z_n$. I am not clear on this point because it seems like you are saying two things in your explanation: 1) You concatenate embeddings of $z_n$ choices with the inter-attention output. 2) You also seem to say that the output probability is not just defined over the target words but the cross product of target words and the $z$ vocabulary.}

%The disadvantage of using such design scheme lies in two aspects. First, the translation quality is deteriorated. Second, the diverse translation by manipulating $\mathbf{z}$ becomes progressively inaccurate as given a sequence $\mathbf{z}$, it might never be trained with any target sentence.


%Therefore, during inference, when $\mathbf{y}_{<n}$ is predicted, we can exhaustively search for $\mathbf{z}_n$ since it does not depend on any previous latent state. The time complexity for searching latent sequence $\mathbf{z}$ drops from $N^{|V_{\mathbf{z}}|}$ to $N|V_{\mathbf{z}}|$.

%Therefore, during inference, 
%when $\mathbf{y}_{<n}$ is predicted, we can exhaustively search for $\mathbf{z}_n$ \rev{because getting $\mathbf{z}_n$ does not depend on any previous latent state. The time complexity for searching latent sequence $\mathbf{z}$ drops from $N^{|V_{\mathbf{z}}|}$ to $N|V_{\mathbf{z}}|$.}  \nb{Xuewen, the previous sentence is confusing. Can you try to restate it?}

% \begin{equation}
%     P(\mathbf{y} \vert \mathbf{x}) 
%     = \sum_{\mathbf{z}\in F(\mathbf{z})} P(\mathbf{y} \vert \mathbf{z},\mathbf{x})P(\mathbf{z} \vert \mathbf{x})
% \end{equation}

%Unlike the two-step decoding models, \name \del{is exposed to all possible $\mathbf{z}$ sequences during training} \yr{breaks the sequence into time-independent variables and explore these variables exhaustively}.
%However, instead of two step decoding\footnote{decoding $\mathbf{z}_n$ using $\log P(\mathbf{z}_n \vert \mathbf{z}_{<n}, \mathbf{x})$ and then decoding $\mathbf{y}_n$ using $\log P(\mathbf{y}_n \vert \mathbf{z}_{\leq n}, \mathbf{x}, \mathbf{y}_{<n})$,}~\cite{wang2018tree, wu2017sequence, aharoni2017}, we directly use $\log P(\mathbf{y}_n, \mathbf{z}_{n} \vert \mathbf{x}, \mathbf{y}_{<n})$ as the beam cost for decoding. 
%\xy{To achieve controlled diverse translation, we can just feed different $\mathbf{z}$ sequences to the right branch of the decoder and decode diverse $\mathbf{y}_n$ by directly using $\log P(\mathbf{y}_n \vert \mathbf{z}_{n}, \mathbf{x}, \mathbf{y}_{<n})$ as the beam cost.}

%\nb{Say something about how you can use this to do controlled decoding for diversity.}

\eat{\yr{Our model also can not exhaustively search the whole latent space during the inference. During the training phrase, when $y$ is fixed, our method can exhaustively search the latent space. During the inference phrase, as $y$ is uncertain, we still need beam search $y$. Nevertheless, our method still can explore a much larger space of the latent space. I wander whether exhaustive search will lead to confusion.}\nb{This is a good point. I like adding ``for Latent States'' to the section heading.}}

%We call this model POS tags guided NMT (POST-NMT).

%The proposed model architecture defines an equivalent Bayesian network, which is presented in Figure~\ref{fig:Bayes1}. 
%The latent variable $\mathbf{z}$ is defined as a non-sequential variable. 
%The latent syntax token $\mathbf{z}_n$ is inferred from source sentence $\mathbf{x}$ and the partial translation $\mathbf{y}_{<n}$, but not from partial sequence $\mathbf{z}_{<n}$. This design scheme gives us the advantage of searching full space of latent $\mathbf{z}$ compared with other models similar to Bayesian network designed in Figure~\ref{fig:Bayes1} and ~\ref{fig:Bayes2}, as the search space reduces from $|V_{\mathbf{z}}|^N$ to $N\times |V_{\mathbf{z}}|$, where $|V_{\mathbf{z}}|$ is the size of the vocabulary $V_{\mathbf{z}}$. \yr{change the symbol from $N_{V_{\mathbf{z}}}$ to $|V_{\mathbf{z}}|$.}
%Even though $\mathbf{z}$ is a non-sequential variable, it has implicit sequential property because of the partial translation $\mathbf{y}_{\leq n}$. Besides, 
%\del{The intuition of this design is that partial sequence $\mathbf{y}_{<n}$ and source sentence $\mathbf{x}$ can provide enough information to infer $\mathbf{z}_n$, even tough there is no information from partial sequence $\mathbf{z}_{<n}$.} \yr{move to the front part.}
%Another more straightforward way of defining the translation process is shown in Figure~\ref{fig:Bayes2}. In this graph, the latent variable $\mathbf{z}$ is defined as a sequential variable. The POS tag token $\mathbf{z}_n$ is inferred from source sentence $\mathbf{x}$ and the partial translation $\mathbf{z}_{<n}$. In this work, we choose Figure~\ref{fig:Bayes1} instead of Figure~\ref{fig:Bayes2} for two reasons. First, in Figure~\ref{fig:Bayes2}, the log-likelihood becomes intractable to calculate due to the exponential search space of $\mathbf{z}$. Second, in Figure~\ref{fig:Bayes1}, 


%\begin{figure}
%\centering
%\includegraphics[width=0.45\textwidth]{bayes.png}
%\caption{Equivalent graphical model of POST-NMT.}
%\label{fig:Bayes}
%\end{figure}



%\subsection{Neural Expectation Maximization}


%This can be maximized by using EM algorithm. 
%In the E step, the lower bound $\mathcal{L}(Q,\boldsymbol{\theta}^{old})$ is maximized with respect to $Q(\mathbf{z})$ while holding $\boldsymbol{\theta}^{old}$ fixed. This will push $Q(\mathbf{z}_n)$ to the posterior distribution $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{<n}; \boldsymbol{\theta}^{old})$, which will push the lower bound $\mathcal{L}_{lower}(Q,\boldsymbol{\theta}^{old})$ close to the log likelihood $\mathcal{L}(\mathbf{\boldsymbol{\theta}}^{old})$. In the subsequent M step, the distribution $Q(\mathbf{z})$ is held fixed and the lower bound $\mathcal{L}(Q,\boldsymbol{\theta})$ is maximized with respect to $\theta$ to give some new value $\boldsymbol{\theta}^{new}$. This will cause the lower bound $\mathcal{L}(Q,\boldsymbol{\theta})$ increase, which will necessarily cause the corresponding log-likelihood function to increase. 
% according to equation~\ref{eq:joint},
% \begin{equation}
% \label{eq:post}
% \begin{aligned}
% P(\mathbf{y}_n, \mathbf{z}_n\vert \mathbf{x}, \mathbf{y}_{<n}) &= P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n}) \\
% &\times P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})
% \end{aligned}
% \end{equation}


%In the remain of this section, we first propose the details of the basic EM for our model. After that, a regularized EM is introduced to incorporate the ground-true POS tag into the training.
%
%\subsection{Neural Expectation Maximization}
%Instead of  $\log P_{\psi}(Y_{1:M}|X_{1:N})$ directly, we optimize the following lower-bound:
%\begin{align}\label{Eq:LB}
%\log &P_{\psi}(Y_{1:M}|X_{1:N}) \geq \sum_{m=1}^{M}\mathcal{Q}_m(\psi_{old}, \psi),\\
%\mathcal{Q}_m&(\psi_{old}, \psi)= \sum_{Z_m}P_{\psi_{old}}(Z_m|Y_m, X_{1:N})\nonumber\\
%&\quad\times \log P_{\psi}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N}),\nonumber
%\end{align}
%where at each time instant, there is a lower bound $\mathcal{Q}_m(\psi_{old}, \psi)$ of the conditional distribution $\log \sum_{Z_m}P_{\psi}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N})$. 
%
%Before proposing the whole training algorithm, we first introduce the training steps at each time slot. At the $m_{th}$ time slot, the EM training of $\mathcal{Q}_m(\psi_{old}, \psi)$ is divided as two following steps:
%
%\noindent\textbf{Expectation (E Step):} In E step, we compute the posterior distribution of $Z_m$ with respect to the current value of the parameter $\psi_{old}$ by
%\begin{align}
%	\gamma&(Z_m=c)=P_{\psi_{old}}(Z_m|Y_m, X_{1:N})\nonumber\\
%	&=\frac{P_{\psi_{old}}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N})}{\sum_{Z_m}P_{\psi_{old}}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N})},
%\end{align}
%where $P_{\psi}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N})$ is given by Eq. (\ref{Eq:Post}). In literature work, $\gamma(Z_m=c)$ is called the responsibility of $Z_m$.
%
%It's not softmax, where softmax needs exponential.
%
%\noindent\textbf{Maximization (M Step):} By substituting the responsibilities, the lower bound $\mathcal{Q}_m(\psi_{old}, \psi)$ is expressed as
%\begin{align*}
%	\mathcal{Q}_m&(\psi_{old}, \psi) = \sum_{c = 1}^{C}\gamma(Z_m=c)\\
%	&\times\log P_{\psi}(Y_{m},Z_{m}|Y_{1:m-1}, X_{1:N}).
%\end{align*}
%In M step, we maximize $\mathcal{Q}_m(\psi_{old}, \psi)$ with respect to $\psi$. As $\mathcal{Q}_m$ is non-convex, closed-form solution $\psi^{\ast}$ is intractable. We update the parameter by gradient method:
%\begin{align*}
%	\psi_{new}=\psi_{old} + \eta \frac{\partial \mathcal{Q}_m(\psi_{old}, \psi)}{\partial \psi},
%\end{align*}
%where $\eta$ is the step-size.
%
%Providing the EM steps at each time slot, the whole training process is given in {\color{red}Algorithm ??}.  


%serves as inferring the latent syntax of the target sentence by clustering the target side tokens into $|V_{\mathbf{z}}|$ different categories. 
%This can make the prediction of $\mathbf{z}_n$ rather inaccurate. 
%As the prediction accuracy of $\mathbf{z}_n$ has significant influence of the translation performance, it is beneficial to regularize the generation of latent sequence $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n})$ with some groundtrue syntax knowledge. In this paper, we consider POS tag sequences of the target sentences extracted by using Stanford Parser \cite{Chen14, Green11} as the syntax knowledge needed.

%In our proposed NEM for POST-NMT model, the prediction accuracy of POS tag for next word has a significant influence of the translation performance. Inaccurate POS tags will lead the translation toward a wrong direction as if the $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n})$ is not accurate enough, the
%$P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})$ will not be accurate either. To reduce the error of POS tag inference and further improve the translation quality, we regularize $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n})$ by the ground-true POS tags of the target sentences extracted by using Stanford Parser \cite{Chen14, Green11}. 


% \subsection{Masked Softmax Layer}
% Similarly to other $seq2seq$ models, we use a learned linear transformation to convert the decoder output to a vocabulary-sized high-level feature and then use a softmax layer to predicted next-token probabilities. Different from theirs which predict the next token from all the vocabulary, in our model, we have to make sure the next predicted token belongs to a specific POS tag. This means that tokens from this POS tag will be given a probability while others will not.  To achieve this, we propose a masked softmax layer. 

% We denote the size of the target vocabulary as $V_y$, the number of POS tag categories is $V_z$, and the output of the linear layer in Figure~\ref{fig:architecture} is $\mathbf{h}$. Then $\mathbf{h}$ is of dimension $B\times S\times V_z \times V_y$. We then create a mask of dimension $V_z \times V_y$ to mask out the words that are not belong to their corresponding POS tags. Then we can calculate a probability based on only the words belong to their corresponding POS tags.

% A mask is first created to make the probability of the words not belonging to the  

% Suppose the size of the target word vocabulary is $N_t$, and the size of the POS tag vocabulary is $N_{pos}$, then the mask is a matrix of size $N_t \times N_{pos}$, with ones on the positions where a specific word belongs to some specific POS tag categories, zeros for others.

%\subsection{Exhaustive Search of Latent Sequences}

%To achieve high translation performance, NMT models usually rely on beam search algorithm for decoding sentences. Beam search finds good candidate translations by considering multiple hypotheses of translations simultaneously. It considers the best $K$ (referred to as \textit{beam size}) hypotheses (i.e., partial translations $P(\mathbf{y}_n\vert \mathbf{x}, \mathbf{y}_{<n})$) in each step, and predicting next output words only for the selected hypotheses. However, in our proposed model, the hidden variable $\mathbf{z}$ has to be taken into consideration. A direct application of beam search in our model is to select the best $K$ hypotheses for $\mathbf{z}$ by $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n})$, then using the best $K$ $z$ to select the best $K$ $y$ by $P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})$. Considering the scenarios where $P(\mathbf{z}_n \vert \mathbf{x}, \mathbf{y}_{< n})$ is low, but $P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})$ is high, we select the best $K$ pairs $(z, y)$ by $P(\mathbf{y}_n, \mathbf{z}_n\vert \mathbf{x}, \mathbf{y}_{<n})$.  

% SRC & danke , dass sie bei ted waren . vielen dank . \\
% REF & thank you so much for coming to ted . thank you . \\
% \midrule
% Transformer & thank you for being at ted . thank you .\\
% \name  & thank you for being at ted . thank you very much .  \\
% \name (groundtrue POS)  & thank you so much for being to ted . thank you .\\
% \midrule
% \midrule
% SRC & es macht großen spaß , auf diese weise musik zu machen , und sie als das 
% publikum haben dann erlebt , wie die musik lebendig kommuniziert . \\
% REF & it is great fun to make music in this way , and you as the audience experienced 
% how music communicates in a lively way . \\
% \midrule
% Transformer & it is a great fun thing to make music in this way , and you have experienced 
% it as the audience , then how music communicates alive .\\
% \name  & it is a lot of fun to make music in this way , and you as the audience experienced 
% how music communicates alive .  \\
% \name (groundtrue POS)  & it is great fun to make music in this way , and you as the audience 
% experienced how music communicates alive .\\
% \midrule
% \midrule
%However, in order to make sure that the translation still capture the main meaning of the source sentence, it starts produce some wrong POS tag sequences. So, our model is kind of making a balance of translation diversity and quality.

%We use \textit{edit distance} ($ED$) to define the distance between two POS tag sequences.
%We evaluate our model's capability to generate diverse translation in two ways. 

%Qualitatively, we pick a single source sentence, use our model to decode the Top-1 sentence and its related POS tag sequence. We then define an edit distance $ED=S$ to the Top-1 POS tag sequence. We sample $10$ POS tag sequences whose edit distance to the Top-1 POS tag sequence equal to $S$. We use these $10$ POS tag sequences to generate new translations and show them in Table~\ref{tab:result-de-en-diverse}.


%This suggests that as is often the case, models with more inductive bias (such as ours) are likely to be more useful in low-data regimes than in large-data ones.
% \subsection{Word}
% See if predicted word belongs to a specific category.

% \subsection{Examples}
% Compare with transformer translation quality. Results shown in Table~\ref{tab:result-de-en-samples}.

% \begin{table*}[!t]
% \caption{Translation examples on IWSLT'14 De-En dataset from our model and the Transformer baseline.}
% \centering
% \small
% \begin{tabular}{cp{12cm}cl}
% \toprule
% SRC & danke , dass sie bei ted waren . vielen dank . \\
% REF & thank you so much for coming to ted . thank you . \\
% \midrule
% Transformer & thank you for being at ted . thank you .\\
% \name  & thank you for being at ted . thank you very much .  \\
% \name (groundtrue POS)  & thank you so much for being to ted . thank you .\\
% \midrule
% \midrule
% SRC & es macht großen spaß , auf diese weise musik zu machen , und sie als das 
% publikum haben dann erlebt , wie die musik lebendig kommuniziert . \\
% REF & it is great fun to make music in this way , and you as the audience experienced 
% how music communicates in a lively way . \\
% \midrule
% Transformer & it is a great fun thing to make music in this way , and you have experienced 
% it as the audience , then how music communicates alive .\\
% \name  & it is a lot of fun to make music in this way , and you as the audience experienced 
% how music communicates alive .  \\
% \name (groundtrue POS)  & it is great fun to make music in this way , and you as the audience 
% experienced how music communicates alive .\\
% \midrule
% \midrule
% SRC & letztes jahr habe ich diese beiden folien gezeigt , um zu veranschaulichen , dass die arktische eiskappe , die für annähernd drei millionen jahre die grösse der unteren 48 staaten hatte , um 40 prozent geschrumpft ist . \\
% REF & last year i showed these two slides so that demonstrate that the arctic ice cap , which for most of the last three million years has been the size of the lower 48 states , has shrunk by 40 percent . \\
% \midrule
% Transformer & last year , i showed these two slides to illustrate that the arctic ice caps that had the size of the lower 48 million states to 40 percent . \\
% \name  & last year , i showed these two slides to illustrate that the arctic ice cap , which for nearly three million years had the size of the lower 48 states , was shrunk by 40 percent .  \\
% \name (groundtrue POS)  & last year i showed these two slides just to illustrate that the arctic ice cap , which for nearly about the last three million years has been the size of the lower 48 states , has shrunk by 40 percent . \\
% \bottomrule
% \end{tabular}
% \label{tab:result-de-en-samples}
% \end{table*}


% experiment ends here

% related work begins here

% Saying far from satisfactory requires point out some 
% fundamental limitation. Let's not get into this. 
%However, methods on how to incorporate syntactic features with NMT are still far from satisfactory though the benefit is enormous as demonstrated in Statistical Machine Translation (SMT)~\cite{Chiang2009, Huang2006, Shen2008}. 
%In training phase, both the source sentence and target sentence are embedded as feature vectors and the model is trained end-to-end with a negative log-likelihood loss.
%Attention-based Neural Machine Translation (NMT) models have shown promising results in various large scale translation tasks~\cite{BahdanauCB14, luong2015, SennrichHB16, Vaswani17}. In training phase, both the source sentence and target sentence are embedded as feature vectors and the model is trained end-to-end with a negative log-likelihood loss. 
%This brings attention-based NMT models a characteristic of simplicity as only a parallel corpus is needed to train a model and then the model tries to learn the latent syntactic relationships of the words by itself. However, with more linguistic tools and techniques advancing, more syntactic or linguistic features like parse trees, part-of-speech tags, and lemmas can be parsed easily and accurately using public semantic parsers~\cite{SLING17, Green11, Chen14}. Thus, how to incorporate these linguistic information into NMT has become a problem worthy to put on efforts, as the benefit of incorporating these features is enormous as shown in Statistical Machine Translation (SMT)~\cite{Chiang2009, Huang2006, Shen2008}.

%The intuition is that with multitask learning, both the translation quality and the performance of POS tagger can be improved. 
%However, this requires careful model selection.
%While our method can also be viewed as a multitask learning process if we regard the POS tagging inference process as an auxiliary task, out translation model is more interpretable as the POS tagging inference results directly guide the translation process and improve the translation quality.
%Shu \textit{et al.}~\shortcite{Shu18} trained two encoder-decoder models, one for generating coarse POS tag sequence of the target sentence using source sentence, the other for generating target sentence based on the generated POS tags and the source sentence. However, the length of the coarse POS tag sequence generated limited structure of the generated sentence. For long target sentence, the short POS tag sequence might not be sufficient enough to model its structure. 
%Others~\cite{gu2018top, wang2018tree, wu2017sequence, aharoni2017}. 



%Incorporating linguistic knowledge into machine translation has been extensively studied in Statistic Machine Translation (SMT) \cite{Chiang2009, Huang2006, Shen2008}. \cite{Shen2008} proposed a target dependency language model for decoder to exploit long distance word relations in SMT using a string-to-dependency algorithm. \cite{Chiang2009} studied how to add a large number of new features to improve syntax-based machine translation system using discriminative training. They discovered that certain new features can improve the performance even of top-scoring MT systems. \cite{Huang2006} proposed a relabeling strategies to add additional information onto the PTB trees to improved MT quality. These methods demonstrated that syntactic or other source-target information can greatly improve MT performance.

%In the previous several years, the  However, in most existing NMT models, the decoded words are not predictable and the decoding process is hard to interpret because of the absence of interaction with external knowledge. Some efforts have been done to either integrating external knowledge into NMT or try to make decoding guided by some external information \cite{chatterjee2017, hasler2018, zhang2018}. But they use external information to guide decoding process when training is done. In training process, the external information is not used to help improve translation quality.





%Part-of-speech (POS) tags can help in language disambiguation. Using POS tags to help improve the quality of translation has been widely studied. In Statistical Machine Translation (SMT), Ueffing \textit{et al.}~\shortcite{Ueffing03} makes use of POS tags and maximum entropy modeling to help translate from English into languages with a highly inflected morphology. In order to enrich the English verbs with the needed information, the authors applied POS tags to English to identify English verbs. While in our work, we directly infer POS tags of target language and use this information to help in translation, which is more challenging and reasonable. Niehues \textit{et al.}~\shortcite{niehues2009} use POS tags to help to model word re-ordering between languages. These methods only use POS tags to help to improve part of translation like the re-ordering problem or enriching verb information, while in our model, POS tags are given more responsibility to not only enrich language information but help to guide the translation process. 



%However, most of the NMT systems learn from raw, sentence-aligned parallel text and use little in the way of external linguistic information or grammars \cite{SennrichLinguistic16}. The extensive use of linguistic resources such as part-of-speech (POS) tags are very common in SMT and yielded better performance. However, usage of such linguistic annotations in NMT has been left under-explored. Works in Neural Machine Translation (NMT) that integrate POS-tags or other linguistic features mostly include two ways. The first is by using feature concatenation. Sennrich \textit{et al.}~\shortcite{SennrichLinguistic16} explored linguistic features like lemmas, subword tags, morphological features, POS tags and dependency labels and concatenate them with sentence features to improve translation quality. Similar work is done by Morishita \textit{et al.} ~\shortcite{Morishita18} that the authors incorporated hierarchical subword features in the encoder to improve translation quality. The second is by Multitask Learning, where a unified multitask NMT model is proposed and then the encoder or attention is shared between various tasks like POS tagging, named-entity recognition, syntactic parsing or semantic parsing ~\cite{Baniata18, Niehues17, Zaremoodi18}. The intuition is that with Multitask learning, both the translation quality and the performance of POS tagger can be improved. However, in these methods, the integration of many auxiliary tasks will make the model inefficient and cubersome. Moreover, how the linguistic information like POS tags help to improve the translation process is never studied explicitly. While our method can also be viewed as a multitask learning process if we regard the POS tagging inference process as an auxiliary task, out translation model is more interpretable as the POS tagging inference results directly guide the translation process and improve the translation quality. 

% related work ends here





%\yr{Compared with the structures of Figure \ref{fig:Bayes1} and \ref{fig:Bayes2}, we preserve merely the links from $y_{<n}$ to $z_n$, and discard the links between $z_n$ as well as the links from $z_{<n}$ to $y_n$. As syntax are already presented in the translation content, $y_{<n}$ and $z_{<n}$ contains duplicated information on predicting $z_n$. Therefore, links between $z_n$ are unnecessary.[It is better to give a reason why we discard the red edges.]}


%Moreover, this limited exploration of the syntactic choices mean that this model 
%decode from a diverse set of $\mathbf{z}$ sequences, 

%Second, it is difficult to realize control the translation by explicitly specifying values for the latent variables because of divergence from training.\yr{???}
%computationally expensive, while alsin errors during both training and inference.

%This can be represented by Figure~\ref{fig:Bayes1}, where two decoders are used to decode the syntax and the semantics. However, sampling of sequence $\mathbf{z}$ is nearly impossible as it involves exponential search. To solve this problem, a general idea is to sample a subset of the full space, which is still computationally costly and also introduce error in both training and inference.

%introduce an additional sequence of variables $\mathbf{z}$ to model syntactic information of the target tokens during decoding. This sequence can model the syntactic choices (or any word-level linguistic information) at each time step.


%model parts-of-speech information of the target sentence but it can be used to model any linguistic information that can be expressed at a word-level. 
%These syntactic choices can be incorporated into the decoding process in multiple ways. One standard way is to let the word choices at each time step depend on the syntactic choices at that time step. This approach, shown in Figure~\ref{fig:Bayes2}, can be easily incorporated into standard sequence-to-sequence models by adding an extra sequence layer, say an LSTM layer, in the decoder that feeds into the original word sequence LSTM layer. However, this is

%An ideal model should capture \yr{all} the co-dependence between syntax and semantics. In particular, for a sequential translation process, the word choice at a time step depends on both the semantics and the syntax of the words generated thus far. Similarly, the syntactic choice at a time step also depends on both semantics and syntax of the previous time steps. \xy{This can be represented by Figure~\ref{fig:Bayes1}, where two decoders are used to decode the syntax and the semantics. However, sampling of sequence $\mathbf{z}$ is nearly impossible as it involves exponential search. To solve this problem, a general idea is to sample a subset of the full space}, \yr{which is still computationally costly and also introduce error in both training and inference.}

%Some of the current research \yr{!!!cite} use a simple way to model this dependence, as shown in Figure~\ref{fig:Bayes2}, where the syntactic choices are modeled using observed sequential variables. However, this is limiting in two ways. First, \yr{this method still} does not allow for full exploration of the space $\mathbf{z}$. The model must use greedy or beam search decoding on the space before decoding the words. 
%Second, it is difficult to realize control the translation by explicitly specifying values for the latent variables because of divergence from training.\yr{???}

%Instead, we propose a model which allows exhaustive search over the latent space, as shown in Figure~\ref{fig:Bayes3}. \yr{Compared with the structures of Figure \ref{fig:Bayes1} and \ref{fig:Bayes2}, we preserve merely the links from $y_{<n}$ to $z_n$, and discard the links between $z_n$ as well as the links from $z_{<n}$ to $y_n$. As syntax are already presented in the translation content, $y_{<n}$ and $z_{<n}$ contains duplicated information on predicting $z_n$. Therefore, links between $z_n$ are unnecessary.[It is better to give a reason why we discard the red edges.]}



%One standard way to model this is to use a stacked sequence model, where the lower layer models the syntactic choices using a latent sequence (\mathbf{z}), and an upper layer that models the word choices conditioned on the input and the syntactic choice at a time 

%Thus the joint probability, $P(\mathbf{y}, \mathbf{z}|\mathbf{x})$, can be specified in terms of the word and syntactic choices at each time step. This joint can be factorized in multiple ways. One standard approach is to condition the 

%In this work, we model the syntactic constraints at any time step as a distribution over the part-of-speech labels using a latent variable.

%Under this model, the output is now additionally conditioned on the latent sequence, which itself is conditioned on the input.

%In this section, we propose our POS tags guided NMT (POST-NMT) and the training algorithm - Regularized Neural Expectation Maximization (RNEM).

%\section{POS Guided Attention Machine Translation}
%{\color{red}
%I leave this part to you, basically you have to define the following things:
%\begin{enumerate}
%	\item $P_{\psi}(Z_{m}|X_{1:N})$ $\rightarrow$ Attention Model for POS Tagging?
%	\item $P_{\psi}(Y_{m}|Z_{m}, Y_{1:m-1}, X_{1:N})$ $\rightarrow$ Attention Model for translation?
%	\item My English is not good. Also, I neglect a lot of details of EM and simply describe the essential part. I think this is not a paper for EM but for your idea on Grammar based translation. So if the section 4 is hard to understand, you can change the expression.
%\end{enumerate}
%
%}

%\subsection{Integrating POS Tags}
%\nb{I stopped here. Will look again in the morning.} 
%\nb{We need a couple of sentences here that motivate the specific way you are using the latents here.}
%Formally, we define the conditional probability of the output at each step as follows:

%we assume $P(\mathbf{y} \vert \mathbf{x})$ involves two choices in this latent sequence model: first, a choice of the latent sequence $\mathbf{z}_1, \ldots , \mathbf{z}_N$ of the target sentence; second, a choice of the words $\mathbf{y}_1, \ldots , \mathbf{y}_N$. We continue to assume that there is some distribution $P(\mathbf{z}_n\vert \mathbf{x}, \mathbf{y}_{<n})$ that models the conditional distribution of the latent variable at time step $n$ conditioned on the source sentence $\mathbf{x}$ and the partial translation $\mathbf{y}_{<n}$. Then depending on this, we can continue to model the distribution $P(\mathbf{y}_{n} \vert \mathbf{z}_n, \mathbf{x}, \mathbf{y}_{<n})$, \textit{i.e.}, the conditional probability of the target word at time step $n$ conditioned on the source sentence, latent variable at time step $n$ and the partial translation $\mathbf{y}_{<n}$. Finally, we are able to model the distribution 




%Target-side baselines include Discrete Structural Planning NMT (DSP-NMT)~\cite{Shu18}
%Tree-decoder~\cite{wang2018tree} IWSLT16 200K DATA DE-EN 32.65

%WMT16 en-de  BiRNN+GCN~\cite{bastings2017graph} test15, test16 23.9
%WMT16 EN-DE 27.8/29.0 BASELINE/SNMT-CCG~\cite{nadejde2017predicting}
%bpe2tree~\cite{aharoni2017} WMT16 test on newstest15 28.7, newstest16 33.24


%variational
%AEVNMT~\cite{Eikema2018} iwslt14 en-de 23.9 de-en 29.3
%source-side
%~\cite{SennrichLinguistic16} re-implement using Transformer
%~\cite{Morishita18} used the IWSLT 2016 training set for the training models, tst2012 as the development set, and tst2013 and tst2014 as the test sets  de-en 30.11  en-de 25.28, fr-en 37.94, en-fr 38.61
%vanilla
%Muti-Agent~\cite{Yiren18} IWSLT14 de-en base-34.70 base standard 33.42, big 35.44, big standard 34.01  en-de 27.89, 28.99, 27.95, 29.52
%WMT14 EN-DE standard 28.4, 30.05, WMT16, 17, 18 SINGLE, 40.68 33.47 48.89, ENSEMBLE 41.23 34.01 49.61
%Layer-Wise~\cite{Tianyu19} IWSLT14 DE-EN   WMT14 EN-DE 4.5m FOR TRAINING NEWSTEST2014 FOR TEST
%AC+LL~\cite{bahdanau2016actorcritic} 28.53 de-en
%AC+LL~\cite{bahdanau2016actorcritic} 28.53 de-en
%iwslt14 de-en Dual Transfer Learning~\cite{Wang18dual} 32.35
%~\cite{denkowski2017} iwslt14 en-fr 34.8
%Edinburgh MT~\cite{Birch14}test2014 25.50
%ConvS2S~\cite{Gehring17} is a entirely convolutional architecture for sequence to sequence machine translation. The model is equipped with gated linear units and residual connections, and uses attention in every decoder layer. The hierarchical structure provides convseq2seq a shorter path to capture long-range dependencies compared to the chain structure modeled by recurrent networks.
%MTL-NMT~\cite{Niehues17} is a Multi-task learning algorithm trained simultaneously on part-of-speech tagging, named entity recognition and machine translation tasks.
%Transformer~\cite{Vaswani17} is a simple network architecture relies entirely on self-attention mechanism to compute representations of the input and output without using RNNs or convolution.
%Show the results for the second choice and the third choice.


%This hybrid decoding thus gives an extra advantage over the other models using two RNNs to model Figure~\ref{fig:Bayes1} and ~\ref{fig:Bayes2}. The decoder is updated in order to maximize the conditional probability of the correct next word as well as to maximize the conditional probability of the correct syntax token, which is a novel training signal.

%The For self-attention inside the encoder layer, $Q,K,V \in \mathcal{R}^{M\times d_{model}}$, while for the self-attention inside the decoder layer, $Q,K,V \in \mathcal{R}^{N\times d_{model}}$, where $M$ and $N$ is the length of the source and target sentence. For inter-attention, which is the attention cross the encoder and decoder from the source to the target, $Q \in \mathcal{R}^{N\times d_{model}}$, $K,V \in \mathcal{R}^{M\times d_{model}}$. All the $Q$, $K$, $V$ come from the hidden representations of the corresponding encoder/decoder layer, but projected by different parameter matrices: $W_Q$, $W_K$ and $W_V$. The output of the inter-attention layer is then fed into a feed-forward layer, a linear layer and a softmax layer to get the probability for the next tokens. The dimension of the output of the whole model becomes $N \times D$, where $D$ is the vocabulary size of the target language.


%The output dimension of the left branch of the decoder is $N \times N_{V_{\mathbf{z}}}$. For the right branch, suppose the hidden states of the inter attention is $h_{\mathbf{y}}\in \mathcal{R}^{N\times d_{model}}$ and the embeddings of all the choices of $\mathbf{z}_n$ is $h_{\mathbf{z}}\in \mathcal{R}^{N_{V_{\mathbf{z}}}\times d_{model}}$, then the add operation produces a hidden state $h = h_{\mathbf{y}} + h_{\mathbf{z}} \in \mathcal{R}^{N\times N_{V_{\mathbf{z}}} \times d_{model}}$.
%The proposed hybridization of the decoder gives us an extra advantage over the other models using two RNNs to model Figure~\ref{fig:Bayes1} and ~\ref{fig:Bayes2}. The decoder is updated in oder to maximize the conditional probability of the correct next word as well as to maximize the conditional probability of the correct syntax token, which is a novel training signal.
